Rational design of nanoscale stabilized oxide catalysts for OER with OC22

The efficiency of $H_2$ production via water electrolysis is typically limited to the sluggish oxygen evolution reaction (OER). As such, significant emphasis has been placed upon improving the rate of OER through the anode catalyst. More recently, the Open Catalyst 2022 (OC22) framework has provided a large dataset of density functional theory (DFT) calculations for OER intermediates on the surfaces of oxides. When coupled with state-of-the-art graph neural network models, total energy predictions can be achieved with a mean absolute error as low as 0.22 eV. In this work, we interpolated a database of the total energy predictions for all slabs and OER surface intermediates for 4,119 oxide materials in the original OC22 dataset using pre-trained models from the OC22 framework. This database includes all terminations of all facets up to a maximum Miller index of 1. To demonstrate the full utility of this database, we constructed a flexible screening framework to identify viable candidate anode catalysts for OER under varying reaction conditions for bulk, surface, and nanoscale Pourbaix stability as well as material cost, overpotential, and metastability. From our assessment, we were able to identify 122 and 68 viable candidates for OER under the bulk and nanoscale regime respectively.

==> sections/future_outlook.tex <==
\subsection{Future outlook}

In order to rapidly assess thousands of candidate materials, we naturally neglected several factors that can influence the development of practical \gls{OER} electrocatalysts. First, our computational methods did not capture the effects of solvation or competition by ubiquitous environmental ions nor did they account for the effect of the electrolyte. This is especially important in the context of seawater electrolysis which is a more naturally abundant feed stock than fresh water, but contains calcium, magnesium, chlorine, and other ions that are detrimental to the catalyst. The high concentration of \ce{Cl^-} in particular will hinder \gls{OER} by competing for active sites to induce \gls{ClER}. This is further compounded by the fact that \ce{Cl^-} selectivity can dissolve the oxide catalyst over time\cite{Vos2019}. A possible direction in the future is to expand our database to include predictions of \gls{ClER} intermediates (\ce{Cl^*} and \ce{ClO^*}) on our oxide catalysts in order to explore \gls{ClER} vs \gls{OER} selectivity. 

Second, we also assumed all catalytic reactions will undergo the simplistic \gls{WNA} mechanism, a four step mechanism originally proposed by\citet{Jaramillo2011} (see Figure~\ref{fig:rxn_pathway}). The \gls{WNA} is the most favorable pathway for Miller indices up to one for \ce{IrO2} and \ce{RuO2} catalysts. However, other mechanisms such as the \gls{I2M} and \gls{LOER} are also possible. \gls{I2M}, which involves a simultaneous adsorption of two \ce{H2O} molecules, has been shown to be favorable on the (011) facet due to the presence of an M-O oxyl radical\cite{Gonzalez2021} which can lead to improved overpotentials. Meanwhile, the \gls{LOER} mechanism is a type of \gls{MvK} reaction whereby lattice oxygen sites at the surface will play a role on forming \ce{OOH*} and desorbing into \ce{O2}, leaving behind a surface vacancy. Therefore another possible expansion to our database is to also explore these alternative reaction mechanisms for \gls{OER}.

Lastly, we emphasize that there is no kinetic information regarding the transition state barriers required to proceed along each reaction step. All assessments of the reaction diagrams are purely thermodynamic and the overpotential itself is also a thermodynamic quantity. As such, information regarding the rate of the reaction is unknown. Despite this, the overpotential has been shown repeatedly to be an excellent measure of experimental activity\cite{Jaramillo2011}.


==> tables/candidates_basic.tex <==
\begin{table}[ht!]
\caption{\label{tab:best_facets_table_5} Summary of screening criteria for candidate catalyst materials for \gls{OER} without considering facet stability on the Wulff shape (continued).}

\begin{tabular}{c|c|c|c}
\hline
\hline
 & & & Cost\\
Formula & facets & $\eta$ (V) & (\$/kg)\\
\hline
\hline

\ce{Ca(FeO2)2} & 2 & 0.40 & 1.90\\
\hline
\ce{PbO2} & 3 & 0.47 & 2.41\\
\hline
\ce{PbO2} & 5 & 0.41 & 2.41\\
\hline
\ce{Cd2PbO4} & 2 & 0.51 & 2.59\\
\hline
\ce{Zn2SiO4} & 2 & 0.48 & 2.79\\
\hline
\ce{Cu3O4} & 2 & 0.50 & 7.89\\
\hline
\ce{CrSbO4} & 2 & 0.44 & 10.19\\
\hline
\ce{LiSbO3} & 2 & 0.62 & 10.82\\
\hline
\ce{CoPbO3} & 3 & 0.41 & 11.78\\
\hline
\ce{Co(SbO3)2} & 2 & 0.66 & 17.18\\
\hline
\ce{Co(NiO2)4} & 2 & 0.63 & 18.53\\
\hline
\ce{Cu3Mo2O9} & 2 & 0.52 & 19.31\\
\hline
\ce{ZnCoO3} & 2 & 0.47 & 19.81\\
\hline
\ce{NiBiO3} & 4 & 0.47 & 20.66\\
\hline
\ce{Ni(BiO3)2} & 2 & 0.40 & 20.88\\
\hline
\ce{CaBi4O9} & 2 & 0.43 & 21.36\\
\hline
\ce{Bi4O7} & 4 & 0.45 & 22.67\\
\hline
\ce{Co(BiO3)2} & 2 & 0.47 & 24.34\\
\hline
\ce{NaBi5O8} & 2 & 0.49 & 27.24\\
\hline
\ce{Co3BiO8} & 2 & 0.50 & 29.01\\
\hline
\ce{Li7Co5O12} & 3 & 0.41 & 30.17\\
\hline
\ce{Co2NiO4} & 4 & 0.42 & 30.91\\
\hline
\ce{FeCo9O20} & 6 & 0.44 & 31.63\\
\hline
\ce{Li(CoO2)4} & 3 & 0.42 & 34.31\\
\hline
\ce{Li(CoO2)8} & 3 & 0.57 & 34.60\\
\hline
\ce{CoO2} & 2 & 0.49 & 34.90\\
\hline
\ce{CoO2} & 2 & 0.52 & 34.90\\
\hline
\ce{LiCo5O8} & 2 & 0.57 & 36.77\\
\hline
\ce{Hg2Mo2O7} & 2 & 0.52 & 42.27\\
\hline
\ce{Na(CoO2)3} & 2 & 0.48 & 51.61\\
\hline
\ce{FeSeO5} & 2 & 0.58 & 54.84\\
\hline
\ce{Bi2Se3O10} & 2 & 0.67 & 56.01\\
\hline
\ce{Bi2(SeO3)3} & 2 & 0.45 & 57.07\\
\hline
\ce{CaSeO4} & 2 & 0.49 & 65.09\\
\hline
\ce{K2Sb4O11} & 2 & 0.55 & 115.60\\
\hline
\ce{V2Se2O11} & 4 & 0.44 & 140.61\\
\hline
\ce{K(CoO2)2} & 3 & 0.45 & 205.67\\
\hline
\ce{AgBiO2} & 2 & 0.68 & 279.98\\
\hline
\ce{Ag2W2O7} & 2 & 0.63 & 284.56\\
\hline
\ce{Cd2GeO4} & 2 & 0.59 & 293.62\\
\hline
\ce{AgHgO2} & 2 & 0.48 & 302.98\\
\hline
\ce{Cd(GaO2)2} & 2 & 0.49 & 305.35\\
\hline
\ce{Cu2AgO4} & 3 & 0.42 & 313.38\\
\hline
\ce{In4(SnO4)3} & 2 & 0.74 & 340.41\\
\hline
\ce{AgSnO3} & 2 & 0.63 & 350.79\\
\hline
\ce{CdAgO2} & 2 & 0.58 & 367.40\\
\hline
\ce{CdAgO2} & 3 & 0.61 & 367.40\\
\hline
\ce{In3Cu3O8} & 4 & 0.57 & 377.35\\
\hline
\ce{InCoO3} & 2 & 0.68 & 387.34\\
\hline
\ce{Ag2BiO3} & 2 & 0.66 & 401.94\\
\hline
\ce{CrAgO4} & 2 & 0.60 & 415.28\\
\hline
\ce{CoAgO3} & 3 & 0.41 & 444.63\\
\hline
\ce{NiAgO2} & 2 & 0.67 & 470.73\\
\hline
\ce{Cd(AgO2)2} & 2 & 0.59 & 471.94\\
\hline
\ce{Ge2BiO6} & 2 & 0.47 & 480.24\\
\hline
\ce{TiAg2O3} & 2 & 0.46 & 594.55\\
\hline
\ce{CoGeO3} & 2 & 0.50 & 604.48\\
\hline
\ce{Ag3O4} & 7 & 0.41 & 714.77\\
\hline
\ce{AgO} & 2 & 0.45 & 745.41\\
\hline
\ce{AgO} & 2 & 0.51 & 745.41\\
\hline
\ce{AgO} & 6 & 0.51 & 745.41\\
\hline
\ce{Ag2GeO3} & 2 & 0.53 & 862.25\\
\hline
\ce{AgGeO3} & 2 & 0.56 & 865.42\\
\hline
\ce{CuReO4} & 2 & 0.46 & 1690.40\\
\hline
\ce{Tl2(SbO3)3} & 2 & 0.66 & 2678.15\\
\hline
\ce{Tl2Cr2O7} & 2 & 0.43 & 3928.44\\
\hline
\ce{TlCoO3} & 2 & 0.42 & 3950.09\\
\hline
\ce{TlFeO3} & 2 & 0.50 & 3979.72\\
\hline
\ce{BaTl2O4} & 2 & 0.43 & 4021.08\\
\hline
\ce{LuCoO3} & 2 & 0.46 & 4666.55\\
\hline
\ce{NaTlO2} & 2 & 0.65 & 4751.26\\
\hline
\ce{Tl2O3} & 2 & 0.41 & 5370.69\\
\hline
\hline
\end{tabular}
\end{table}

